AV-CPL: Continuous Pseudo-Labeling for Audio-Visual Speech Recognition

Audio-visual speech contains synchronized audio and visual information that provides cross-modal supervision to learn representations for both automatic speech recognition (ASR) and visual speech recognition (VSR). We introduce continuous pseudo-labeling for audio-visual speech recognition (AV-CPL), a semi-supervised method to train an audio-visual speech recognition (AVSR) model on a combination of labeled and unlabeled videos with continuously regenerated pseudo-labels. Our models are trained for speech recognition from audio-visual inputs and can perform speech recognition using both audio and visual modalities, or only one modality. Our method uses the same audio-visual model for both supervised training and pseudo-label generation, mitigating the need for external speech recognition models to generate pseudo-labels. AV-CPL obtains significant improvements in VSR performance on the LRS3 dataset while maintaining practical ASR and AVSR performance. Finally, using visual-only speech data, our method is able to leverage unlabeled visual speech to improve VSR.

==> tables/audio/audio_main.tex <==
\begin{table*}[t] 
\centering
\caption{Comparison of audio-only semi-supervised methods: self-supervised learning and continuous pseudo-labeling. We reproduced SlimIPL on LRS3. 
\textsuperscript{\textdagger}Results presented in~\cite{shi2022learning}. TD=Transformer Decoder. }
\label{tab:audio-main}
\vspace{-3mm}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccccrrr}
\toprule
\multirow{3}{*}{Method} & \multirow{3}{*}{Model} & Encoder & \multirow{3}{*}{Criterion} & \multirow{3}{*}{TD} & \multicolumn{1}{c}{Labeled} & \multicolumn{1}{c}{Unlabeled} & \multirow{3}{*}{PL Stage}  & \multicolumn{3}{c}{Test WER (\%)} \\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & Size & & \multicolumn{1}{c}{} 
 & \multicolumn{1}{c}{Data} & \multicolumn{1}{c}{Data} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{LM} \\
 \cmidrule{9-11}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} &  & &  &  & &  \multicolumn{1}{c}{} & \multicolumn{1}{c}{None} & \multicolumn{1}{c}{30h} & \multicolumn{1}{c}{433h} \\
\hline
\rowcolor{Gray} \multicolumn{11}{c}{\textit{Supervised}}\\
RAVEn~\citep{haliassos2023jointly} & Transformer & 328M & CTC+CE & \cmark & 30h & - & - & \textbf{9.9} & - & - \\
SlimIPL~\citep{likhomanenko21b_interspeech} & Transformer & 256M & CTC & \xmark & 30h & - & - & 11.1 & 8.0 & \textbf{7.3} \\
\hline
\citet{ma2021end} & Conformer & - & CTC+CE &  \cmark & 433h & - & - & 2.3 & - & - \\
RAVEn~\citep{haliassos2023jointly} & Transformer & 328M & CTC+CE & \cmark & 433h & - & - & \textbf{2.2} & - & - \\
SlimIPL~\citep{likhomanenko21b_interspeech} & Transformer & 256M & CTC & \xmark & 433h & - & - & 2.5 & 2.2 & \textbf{2.1} \\
\hline
\rowcolor{Gray} \multicolumn{11}{c}{\textit{Semi-Supervised}}\\
HuBERT~\citep{hsu2021hubert}\textsuperscript{\textdagger} & Transformer & 300M & CE & \cmark & 30h & 433h & - & 4.5 & - & - \\
SlimIPL~\citep{likhomanenko21b_interspeech} & Transformer & 256M & CTC & \xmark & 30h & 433h & PL LRS3 & 5.2 & 3.6 & 3.2 \\
SlimIPL~\citep{likhomanenko21b_interspeech} & Transformer & 256M & CTC & \xmark & 30h & 433h & +FT LRS3 & \textbf{4.3} & 3.2 & \textbf{3.1} \\
\hline
HuBERT~\citep{hsu2021hubert}\textsuperscript{\textdagger} & Transformer & 300M & CE & \cmark & 30h & 1,759h & - & \textbf{3.2} & - & - \\
SlimIPL~\citep{likhomanenko21b_interspeech} & Transformer & 256M & CTC & \xmark & 30h & 1,759h & PL (Vox + LRS3) & 5.7 & 3.9 & 3.3 \\
SlimIPL~\citep{likhomanenko21b_interspeech} & Transformer & 256M & CTC & \xmark & 30h & 1,326h & PL Vox & 6.3 & 4.3 & 3.9 \\
SlimIPL~\citep{likhomanenko21b_interspeech} & Transformer & 256M & CTC & \xmark & 30h & 1,759h & +PL LRS3 & 4.5 & 3.4 & 3.3 \\
SlimIPL~\citep{likhomanenko21b_interspeech} & Transformer & 256M & CTC & \xmark & 30h & 1,759h & +FT LRS3 & 3.8 & 3.2 & \textbf{3.0} \\
\bottomrule
\end{tabular}%
\vspace{-0.6cm}
}
\end{table*}

==> tables/audio_visual/av_architecture.tex <==
\begin{table}[t!]
\centering
\caption{AVSR architecture comparison with Transformer-Base on 433h LRS3 videos and 433h LM. }
\label{tab:av-architecture}
\vspace{2mm}
\resizebox{0.5\columnwidth}{!}{%
\begin{tabular}{lccrr|rr|rr}
\toprule
Audio & & Mod. & \multicolumn{2}{c}{ASR WER} & \multicolumn{2}{c}{AVSR WER} & \multicolumn{2}{c}{VSR WER} \\
Model & Fusion  & Drop & \multicolumn{1}{c}{Val} & \multicolumn{1}{c}{Test} & \multicolumn{1}{c}{Val} & \multicolumn{1}{c}{Test} & \multicolumn{1}{c}{Val} & \multicolumn{1}{c}{Test} \\
\midrule
Conv. & Concat. & N & 18.7 & 20.0 & 8.5 & 10.1 & 60.4 & 69.6 \\
Conv. & Concat. & Y & 8.0 & 5.9 & 12.7 & 13.5 & 71.3 & 77.4 \\
Conv. & Add & N & 17.9 & 19.6 & \textbf{8.2} & \textbf{9.1} & \textbf{60.2} & \textbf{69.0} \\
Conv. & Add & Y & \textbf{7.8} & 5.7 & 12.2 & 12.3 & 71.3 & 78.0 \\
Linear & Concat. & N & 32.8 & 31.7 & 9.1 & 10.1 & 62.7 & 70.8 \\
Linear & Concat. & Y & 8.0 & \textbf{5.6} & 13.8 & 14.8 & 71.1 & 77.8 \\
Linear & Add & N & 27.7 & 31.3 & 8.6 & 9.4 & 61.1 & 69.4 \\
Linear & Add & Y & 8.6 & 6.0 & 13.9 & 14.4 & 73.0 & 78.1 \\
\bottomrule
\end{tabular}%
}
\vspace{-0.4cm}
\end{table}


==> tables/audio_visual/av_modality_drop.tex <==
\begin{table}[h]
\centering
\caption{Ablation study on audio-visual modality dropout for AV-CPL using LRS3 433h labeled videos and VoxCeleb2 1,326h unlabeled videos with transformer-Base. The first row shows the seed model with $p_m=p_a=0.5$.}
\label{tab:av-mod-drop}
\vspace{2mm}
\resizebox{0.5\columnwidth}{!}{%
\begin{tabular}{rlrr|rr|rr}
\toprule
\multicolumn{1}{c}{Mod.} & \multicolumn{1}{c}{VoxCeleb2} & \multicolumn{2}{c}{ASR WER} & \multicolumn{2}{c}{AVSR WER} & \multicolumn{2}{c}{VSR WER} \\
\multicolumn{1}{c}{Dropout} & \multicolumn{1}{c}{Unlabeled} & \multicolumn{1}{c}{Val} & \multicolumn{1}{c}{Test} & \multicolumn{1}{c}{Val} & \multicolumn{1}{c}{Test} & \multicolumn{1}{c}{Val} & \multicolumn{1}{c}{Test} \\
\multicolumn{1}{l}{$p_m'=p_a'$} & & & & & & & \\
\midrule
Seed & Model & \textbf{2.9} & \textbf{2.6} & \textbf{2.8} & \textbf{2.6} & \textbf{60.7} & \textbf{67.0} \\
\midrule
0.5 & 1,326h & \textbf{3.4} & \textbf{2.2} & \textbf{3.1} & \textbf{2.0} & 46.8 & 55.7 \\
0.25 & 1,326h & 4.0 & 2.7 & 3.9 & 2.5 & 34.0 & 49.9 \\
0.1 & 1,326h & 4.9 & 3.3 & 4.9 & 3.0 & 30.9 & 48.4 \\
0.05 & 1,326h & 5.8 & 4.1 & 5.5 & 4.0 & \textbf{28.2} & \textbf{48.3} \\
\bottomrule
\end{tabular}%
\vspace{-0.4cm}
}
\end{table}

==> tables/audio_visual/av_representation_433h_base_nolm.tex <==
\begin{table}[t!]
\centering
\caption{AVSR modality pre-training ablation with labeled LRS3 433h, Transformer-Base, and 433h LM.}
\label{tab:av-representation-433h-base-nolm}
\vspace{2mm}
\resizebox{0.5\columnwidth}{!}{%
\begin{tabular}{lccrr|rr|rr}
\toprule
Train & & Mod. & \multicolumn{2}{c}{ASR WER} & \multicolumn{2}{c}{AVSR WER} & \multicolumn{2}{c}{VSR WER} \\
Mods. & PT & Drop & \multicolumn{1}{c}{Val} & \multicolumn{1}{c}{Test} & \multicolumn{1}{c}{Val} & \multicolumn{1}{c}{Test} & \multicolumn{1}{c}{Val} & \multicolumn{1}{c}{Test} \\
\midrule
AV & - & N & 13.5 & 15.4 & \textbf{3.3} & \textbf{4.5} & \textbf{56.3} & \textbf{66.7} \\
AV & - & Y & \textbf{4.2} & \textbf{3.0} & 7.8 & 9.6 & 66.4 & 74.6 \\
\midrule
A & - & - & \textbf{2.4} & \textbf{2.4} & 94.1 & 94.8 & 99.9 & 99.9 \\
V & - & - & 99.9 & 99.9 & \textbf{49.8} & \textbf{68.1} & \textbf{49.9} & \textbf{67.7} \\
\midrule
AV & A & N & 3.2 & 3.2 & \textbf{1.9} & \textbf{2.5} & 67.1 & 71.3 \\
AV & A & Y & \textbf{2.9} & \textbf{2.6} & 2.8 & 2.6 & \textbf{60.7} & \textbf{67.0} \\
\midrule
AV & V & N & 92.4 & 85.9 & \textbf{8.7} & \textbf{21.7} & \textbf{39.1} & \textbf{63.8} \\
AV & V & Y & \textbf{5.7} & \textbf{4.7} & 12.3 & 23.5 & 47.2 & 66.7 \\
\bottomrule
\end{tabular}%
}
\vspace{-0.4cm}
\end{table}

==> tables/audio_visual/av_stride.tex <==
\begin{table}[t!]
\centering
\caption{Ablation study on token set (characters and subwords) vs stride for AVSR using labeled LRS3 433h, transformer-Base, and 433h LM.}
\label{tab:av-stride}
\vspace{2mm}
\resizebox{0.5\columnwidth}{!}{%
\begin{tabular}{llrr|rr|rr}
\toprule
\multirow{3}{*}{Tokens} & \multirow{3}{*}{Stride} & \multicolumn{2}{c}{ASR WER (\%)} & \multicolumn{2}{c}{AVSR WER (\%)} & \multicolumn{2}{c}{VSR WER (\%)} \\
 &  & \multicolumn{1}{c}{Val} & \multicolumn{1}{c}{Test} & \multicolumn{1}{c}{Val} & \multicolumn{1}{c}{Test} & \multicolumn{1}{c}{Val} & \multicolumn{1}{c}{Test} \\
 \midrule
Characters & 20ms & \textbf{4.2} & \textbf{3.0} & \textbf{7.8} & \textbf{9.6} & \textbf{66.4} & \textbf{74.6} \\
Characters & 40ms & 7.8 & 5.7 & 12.2 & 12.3 & 71.3 & 78.0 \\
\midrule
Subwords & 20ms & 6.3 & 9.9 & \textbf{5.6} & \textbf{9.7} & 67.6 & 72.4 \\
Subwords & 40ms & \textbf{5.5} & \textbf{7.1} & 8.4 & 14.4 & \textbf{60.6} & \textbf{70.1} \\
\bottomrule
\end{tabular}%
\vspace{-0.4cm}
}
\end{table}

